Evaluating the Faithfulness of Importance Measures in NLP by Recursively Masking Allegedly Important Tokens and Retraining

To explain NLP models a popular approach is to use importance measures, such as attention, which inform input tokens are important for making a prediction. However, an open question is how well these explanations accurately reflect a model's logic, a property called faithfulness. To answer this question, we propose Recursive ROAR, a new faithfulness metric. This works by recursively masking allegedly important tokens and then retraining the model. The principle is that this should result in worse model performance compared to masking random tokens. The result is a performance curve given a masking-ratio. Furthermore, we propose a summarizing metric using relative area-between-curves (RACU), which allows for easy comparison across papers, models, and tasks. We evaluate 4 different importance measures on 8 different datasets, using both LSTM-attention models and RoBERTa models. We find that the faithfulness of importance measures is both model-dependent and task-dependent. This conclusion contradicts previous evaluations in both computer vision and faithfulness of attention literature.

==> chapter/speculation.tex <==
\section{Speculations}
\label{sec:speculation}

% General finding, NFLT
We find that the faithfulness of an importance measure is both model-dependent and task-dependent. Why this is the case, has by far been the most common question asked when talking with other interpretability researchers about this work. With the current understanding of importance measures, it is impossible to give a general answer to why. However, simultaneous theoretical work have show that the No Free Lunch Theorem \citep{Wolpert1996} applies to some importance measures too \citep{Han2022}.

% Attention as a case example
For attention, the faithfulness should depend on the level of input mixing happening in the BiLSTM layer. For example, it is entirely possible for a BiLSTM layer to simply shift all input tokens one time-step to the left. In this case, when attention points at the 2nd token it is the 1st token that is actually important. In such a case, attention would not be faithful. However, if the BiLSTM layer acts more as a dense layer then attention would be faithful. If different tasks cause different model behaviors, the faithfulness of attention will be task-dependent.

% The explanation-interpretation faithfulness gap
Another factor that can discount faithfulness, is the implicit gap between what an explanation says and how we interpret it. For example, the \emph{gradient w.r.t. the input} method must somehow reflect the model, as it depends only on the model and the input. The faithfulness issue therefore happens when we decide to interpret gradient as importance. The faithfulness measures presented in this paper and by \citet{Hooker2019} evaluates the faithfulness of an ``importance'' interpretation via masking. To which degree gradient and importance are the same depends on the model. For example, in a model that is highly non-linear locally or has zero gradient locally, the gradient may have little correlation with importance. Hence, the faithfulness of the importance measure can be both task-dependent and model-dependent.

% Notes:
% Large gap in our fundamental understanding, of what these explanations are showing and what they can and can not be used for. % https://iclr.cc/virtual/2022/invited-talk/7237
% Saliency maps contain network ``fingerprints'' - can tell which model an explanation comes from.

Regardless of whether or not these hypotheses are true, the model-dependent and task-dependent conclusion makes it necessary to always evaluate the faithfulness of importance measures.


==> table/riemann_samples.tex <==
\begin{tabular}{llllrrrrr}
\toprule
       &     &              & {} & \multicolumn{5}{l}{rank-error} \\
       &     &              & ranks &        all &       c-1 &      c-10 &      q-10 &      q-90 \\
dataset & samples & walltime & abs_error &            &           &           &           &           \\
\midrule
\multirow{12}{*}{Anemia} & 2   & 101.245534   & 4.212499e-04 &   0.981569 &  0.359217 &  0.670127 &  0.931639 &  0.985561 \\
       & 5   & 224.211633   & 1.900731e-04 &   0.952694 &  0.223809 &  0.486668 &  0.854859 &  0.962467 \\
       & 10  & 465.211974   & 9.743480e-05 &   0.910150 &  0.165410 &  0.361784 &  0.763002 &  0.926461 \\
       & 20  & 855.312985   & 4.272683e-05 &   0.822572 &  0.085673 &  0.223873 &  0.594393 &  0.846262 \\
       & 30  & 1288.854942  & 2.567901e-05 &   0.732999 &  0.060966 &  0.158623 &  0.469494 &  0.759835 \\
       & 40  & 1917.144134  & 1.705118e-05 &   0.639946 &  0.044120 &  0.118931 &  0.370341 &  0.666477 \\
       & 50  & 2416.830668  & 1.156951e-05 &   0.543600 &  0.032087 &  0.088545 &  0.285903 &  0.567741 \\
       & 60  & 2808.785240  & 8.211632e-06 &   0.448582 &  0.030002 &  0.076207 &  0.224991 &  0.469050 \\
       & 70  & 2816.397905  & 5.715537e-06 &   0.350925 &  0.023584 &  0.063084 &  0.170533 &  0.366898 \\
       & 80  & 3215.318586  & 3.986991e-06 &   0.253103 &  0.021980 &  0.057292 &  0.127318 &  0.264332 \\
       & 90  & 3450.266509  & 2.162507e-06 &   0.146725 &  0.016044 &  0.041778 &  0.079742 &  0.152731 \\
       & 100 & 4290.197410  & 0.000000e+00 &   0.000000 &  0.000000 &  0.000000 &  0.000000 &  0.000000 \\
\cline{1-9}
\multirow{12}{*}{Diabetes} & 2   & 216.577702   & 3.693328e-04 &   0.987038 &  0.039321 &  0.414004 &  0.932146 &  0.987547 \\
       & 5   & 493.015442   & 1.226521e-04 &   0.969338 &  0.019529 &  0.265596 &  0.883182 &  0.970705 \\
       & 10  & 1044.036231  & 5.613671e-05 &   0.939109 &  0.011348 &  0.161049 &  0.811889 &  0.941372 \\
       & 20  & 2131.249034  & 2.473134e-05 &   0.876072 &  0.006422 &  0.085125 &  0.690026 &  0.879103 \\
       & 30  & 3037.823552  & 1.438819e-05 &   0.808189 &  0.004662 &  0.054249 &  0.582591 &  0.811228 \\
       & 40  & 4094.933739  & 9.237436e-06 &   0.735016 &  0.003519 &  0.036348 &  0.484113 &  0.737431 \\
       & 50  & 5792.294085  & 6.153519e-06 &   0.655240 &  0.003167 &  0.025255 &  0.393797 &  0.656560 \\
       & 60  & 6408.906722  & 4.100251e-06 &   0.567722 &  0.002903 &  0.018174 &  0.309460 &  0.567615 \\
       & 70  & 6668.413624  & 2.634924e-06 &   0.469620 &  0.002375 &  0.012201 &  0.229474 &  0.467858 \\
       & 80  & 7265.292086  & 1.536612e-06 &   0.356380 &  0.002199 &  0.007855 &  0.152747 &  0.352923 \\
       & 90  & 9419.508060  & 6.827888e-07 &   0.216496 &  0.001319 &  0.004601 &  0.077924 &  0.212074 \\
       & 100 & 10339.881488 & 0.000000e+00 &   0.000000 &  0.000000 &  0.000000 &  0.000000 &  0.000000 \\
\cline{1-9}
\multirow{12}{*}{IMDB} & 2   & 43.092894    & 1.037579e-02 &   0.871993 &  0.085208 &  0.391808 &  0.499771 &  0.866614 \\
       & 5   & 89.239690    & 4.029346e-03 &   0.744075 &  0.035474 &  0.207157 &  0.302828 &  0.735468 \\
       & 10  & 171.989350   & 1.917285e-03 &   0.587424 &  0.017389 &  0.110913 &  0.177513 &  0.576848 \\
       & 20  & 330.252559   & 8.541130e-04 &   0.390915 &  0.007806 &  0.053173 &  0.089459 &  0.380840 \\
       & 30  & 475.414340   & 4.986248e-04 &   0.273621 &  0.004367 &  0.031417 &  0.054708 &  0.265358 \\
       & 40  & 635.290816   & 3.206723e-04 &   0.195633 &  0.002782 &  0.020326 &  0.035992 &  0.189241 \\
       & 50  & 841.868045   & 2.138323e-04 &   0.139993 &  0.001778 &  0.013224 &  0.024141 &  0.135105 \\
       & 60  & 985.008599   & 1.425776e-04 &   0.098242 &  0.001237 &  0.008811 &  0.016144 &  0.094659 \\
       & 70  & 1141.382244  & 9.166776e-05 &   0.065693 &  0.000657 &  0.005750 &  0.010543 &  0.063223 \\
       & 80  & 1284.326926  & 5.347724e-05 &   0.039502 &  0.000232 &  0.003215 &  0.006170 &  0.037963 \\
       & 90  & 1467.748873  & 2.376944e-05 &   0.017988 &  0.000077 &  0.001465 &  0.002712 &  0.017278 \\
       & 100 & 1628.388538  & 0.000000e+00 &   0.000000 &  0.000000 &  0.000000 &  0.000000 &  0.000000 \\
\cline{1-9}
\multirow{12}{*}{SNLI} & 2   & 128.844450   & 3.029601e-02 &   0.678536 &  0.206067 &  0.630414 &  0.235966 &  0.676351 \\
       & 5   & 201.026176   & 9.867780e-03 &   0.409434 &  0.076203 &  0.354065 &  0.092569 &  0.407639 \\
       & 10  & 310.218702   & 4.700520e-03 &   0.251190 &  0.036740 &  0.206646 &  0.045774 &  0.249090 \\
       & 20  & 541.730724   & 2.104439e-03 &   0.132711 &  0.016549 &  0.104526 &  0.020897 &  0.130988 \\
       & 30  & 799.702943   & 1.230916e-03 &   0.082936 &  0.009623 &  0.064042 &  0.012232 &  0.081641 \\
       & 40  & 1138.658037  & 7.923950e-04 &   0.055321 &  0.006170 &  0.042151 &  0.007891 &  0.054385 \\
       & 50  & 1382.009402  & 5.287155e-04 &   0.037886 &  0.004151 &  0.028631 &  0.005320 &  0.037201 \\
       & 60  & 1497.165611  & 3.526816e-04 &   0.025691 &  0.002752 &  0.019303 &  0.003556 &  0.025202 \\
       & 70  & 1719.830389  & 2.268183e-04 &   0.016698 &  0.001698 &  0.012468 &  0.002208 &  0.016348 \\
       & 80  & 2233.465927  & 1.323520e-04 &   0.009890 &  0.000984 &  0.007363 &  0.001277 &  0.009679 \\
       & 90  & 2445.198340  & 5.883791e-05 &   0.004465 &  0.000446 &  0.003319 &  0.000570 &  0.004380 \\
       & 100 & 2595.697045  & 0.000000e+00 &   0.000000 &  0.000000 &  0.000000 &  0.000000 &  0.000000 \\
\cline{1-9}
\multirow{12}{*}{SST} & 2   & 6.179342     & 4.125003e-02 &   0.345318 &  0.063566 &  0.273893 &  0.097015 &  0.346495 \\
       & 5   & 10.537298    & 1.616349e-02 &   0.171881 &  0.026513 &  0.126903 &  0.041160 &  0.172109 \\
       & 10  & 11.270489    & 7.688394e-03 &   0.090985 &  0.012387 &  0.063882 &  0.019260 &  0.090847 \\
       & 20  & 14.584255    & 3.424350e-03 &   0.043213 &  0.005868 &  0.029249 &  0.009417 &  0.042925 \\
       & 30  & 19.207759    & 1.998944e-03 &   0.025854 &  0.003151 &  0.016976 &  0.005053 &  0.025529 \\
       & 40  & 23.707140    & 1.285492e-03 &   0.016397 &  0.002391 &  0.010675 &  0.003405 &  0.016165 \\
       & 50  & 27.695689    & 8.571772e-04 &   0.011072 &  0.001630 &  0.007465 &  0.002427 &  0.011019 \\
       & 60  & 33.658953    & 5.715312e-04 &   0.007224 &  0.001087 &  0.004852 &  0.001612 &  0.007185 \\
       & 70  & 38.382564    & 3.674495e-04 &   0.004556 &  0.000543 &  0.003181 &  0.000851 &  0.004546 \\
       & 80  & 40.515218    & 2.143618e-04 &   0.002636 &  0.000435 &  0.001813 &  0.000525 &  0.002616 \\
       & 90  & 48.007606    & 9.527827e-05 &   0.001150 &  0.000217 &  0.000788 &  0.000290 &  0.001149 \\
       & 100 & 48.787989    & 0.000000e+00 &   0.000000 &  0.000000 &  0.000000 &  0.000000 &  0.000000 \\
\cline{1-9}
\multirow{12}{*}{bAbI-1} & 2   & 7.425629     & 1.081415e-01 &   0.851283 &  0.249364 &  0.718864 &  0.453836 &  0.847859 \\
       & 5   & 8.124638     & 3.858272e-02 &   0.690323 &  0.163909 &  0.503700 &  0.307677 &  0.684464 \\
       & 10  & 10.991558    & 1.176209e-02 &   0.450357 &  0.063091 &  0.254918 &  0.148500 &  0.442510 \\
       & 20  & 13.864422    & 2.284346e-03 &   0.203838 &  0.013818 &  0.080291 &  0.042392 &  0.197764 \\
       & 30  & 17.867403    & 7.844175e-04 &   0.099069 &  0.005000 &  0.029945 &  0.014994 &  0.094974 \\
       & 40  & 23.031856    & 3.776491e-04 &   0.050868 &  0.002727 &  0.014027 &  0.006545 &  0.048273 \\
       & 50  & 30.729127    & 2.219148e-04 &   0.029322 &  0.001364 &  0.007718 &  0.003698 &  0.027720 \\
       & 60  & 30.525028    & 1.401889e-04 &   0.017799 &  0.000818 &  0.004473 &  0.002283 &  0.016772 \\
       & 70  & 36.853598    & 8.827613e-05 &   0.011075 &  0.000455 &  0.002809 &  0.001252 &  0.010478 \\
       & 80  & 41.546208    & 5.110717e-05 &   0.006300 &  0.000273 &  0.001645 &  0.000945 &  0.005965 \\
       & 90  & 44.202871    & 2.296823e-05 &   0.003196 &  0.000273 &  0.000864 &  0.000521 &  0.003037 \\
       & 100 & 45.209531    & 0.000000e+00 &   0.000000 &  0.000000 &  0.000000 &  0.000000 &  0.000000 \\
\cline{1-9}
\multirow{12}{*}{bAbI-2} & 2   & 15.312163    & 2.878886e-01 &   0.957670 &  0.535091 &  0.871600 &  0.824966 &  0.956850 \\
       & 5   & 19.680807    & 2.724161e-01 &   0.939688 &  0.437727 &  0.816827 &  0.766893 &  0.938413 \\
       & 10  & 27.398557    & 1.840523e-01 &   0.911351 &  0.343909 &  0.745300 &  0.695440 &  0.909493 \\
       & 20  & 45.474422    & 1.289366e-01 &   0.867509 &  0.265364 &  0.658391 &  0.615779 &  0.865040 \\
       & 30  & 64.054374    & 1.165800e-01 &   0.836549 &  0.239727 &  0.612045 &  0.577744 &  0.833669 \\
       & 40  & 77.930287    & 9.688232e-02 &   0.811348 &  0.211636 &  0.573982 &  0.541338 &  0.808298 \\
       & 50  & 104.210327   & 6.895255e-02 &   0.773628 &  0.146636 &  0.502655 &  0.476521 &  0.769994 \\
       & 60  & 131.502538   & 8.642209e-02 &   0.772235 &  0.191909 &  0.530418 &  0.505219 &  0.769344 \\
       & 70  & 152.124177   & 8.517199e-02 &   0.757961 &  0.189273 &  0.517764 &  0.495242 &  0.754956 \\
       & 80  & 143.654563   & 7.428072e-02 &   0.738748 &  0.175091 &  0.490282 &  0.470681 &  0.735710 \\
       & 90  & 167.494699   & 8.025901e-02 &   0.728735 &  0.177909 &  0.489391 &  0.470783 &  0.726110 \\
       & 100 & 192.393586   & 0.000000e+00 &   0.000000 &  0.000000 &  0.000000 &  0.000000 &  0.000000 \\
\cline{1-9}
\multirow{12}{*}{bAbI-3} & 2   & 27.774496    & 1.729354e-01 &   0.982463 &  0.562636 &  0.864336 &  0.913653 &  0.981887 \\
       & 5   & 49.460336    & 1.114488e-01 &   0.970721 &  0.410455 &  0.777245 &  0.855408 &  0.969511 \\
       & 10  & 82.138040    & 8.716298e-02 &   0.949756 &  0.295727 &  0.653200 &  0.774445 &  0.947338 \\
       & 20  & 172.415194   & 7.651677e-02 &   0.915627 &  0.216000 &  0.530645 &  0.685473 &  0.911663 \\
       & 30  & 214.012361   & 9.021264e-02 &   0.893471 &  0.216364 &  0.492391 &  0.647871 &  0.888786 \\
       & 40  & 323.617345   & 7.589681e-02 &   0.874283 &  0.192455 &  0.453400 &  0.614128 &  0.869164 \\
       & 50  & 386.221956   & 4.653517e-02 &   0.849599 &  0.133000 &  0.385218 &  0.559955 &  0.843597 \\
       & 60  & 445.447177   & 2.164273e-01 &   0.846893 &  0.180727 &  0.415809 &  0.575162 &  0.840993 \\
       & 70  & 473.667068   & 8.822861e-02 &   0.838317 &  0.197091 &  0.415827 &  0.569455 &  0.832384 \\
       & 80  & 560.828869   & 6.845812e-02 &   0.825183 &  0.176818 &  0.392682 &  0.548454 &  0.818878 \\
       & 90  & 630.839226   & 8.787030e-01 &   0.819522 &  0.184818 &  0.395764 &  0.548138 &  0.813215 \\
       & 100 & 726.316175   & 0.000000e+00 &   0.000000 &  0.000000 &  0.000000 &  0.000000 &  0.000000 \\
\bottomrule
\end{tabular}


==> table/sparsity.tex <==
\begin{tabular}{llll}
\toprule
       & {} & \multicolumn{2}{l}{total importance} \\
       & k &                        1  &                         10 \\
dataset & importance measure &                           &                            \\
\midrule
\multirow{3}{*}{Anemia} & Attention &   $1\%^{+1.1\%}_{-0.5\%}$ &    $7\%^{+7.5\%}_{-3.8\%}$ \\
       & Gradient &   $1\%^{+0.2\%}_{-0.2\%}$ &    $6\%^{+1.3\%}_{-1.1\%}$ \\
       & Integrated Gradient &   $2\%^{+0.9\%}_{-0.6\%}$ &   $14\%^{+4.5\%}_{-3.5\%}$ \\
\cline{1-4}
\multirow{3}{*}{Diabetes} & Attention &  $22\%^{+3.6\%}_{-3.2\%}$ &   $53\%^{+5.5\%}_{-5.6\%}$ \\
       & Gradient &   $7\%^{+1.1\%}_{-1.0\%}$ &   $32\%^{+2.7\%}_{-2.6\%}$ \\
       & Integrated Gradient &  $18\%^{+1.6\%}_{-1.5\%}$ &   $43\%^{+3.4\%}_{-3.3\%}$ \\
\cline{1-4}
\multirow{3}{*}{IMDB} & Attention &   $9\%^{+2.2\%}_{-1.8\%}$ &   $43\%^{+9.9\%}_{-9.4\%}$ \\
       & Gradient &   $3\%^{+0.5\%}_{-0.4\%}$ &   $20\%^{+3.1\%}_{-2.7\%}$ \\
       & Integrated Gradient &   $9\%^{+1.1\%}_{-1.0\%}$ &   $39\%^{+2.7\%}_{-2.6\%}$ \\
\cline{1-4}
\multirow{3}{*}{SNLI} & Attention &  $38\%^{+1.3\%}_{-1.3\%}$ &   $95\%^{+0.5\%}_{-0.5\%}$ \\
       & Gradient &  $31\%^{+0.5\%}_{-0.5\%}$ &   $93\%^{+0.3\%}_{-0.3\%}$ \\
       & Integrated Gradient &  $28\%^{+0.9\%}_{-0.9\%}$ &   $91\%^{+0.2\%}_{-0.2\%}$ \\
\cline{1-4}
\multirow{3}{*}{SST} & Attention &  $26\%^{+7.4\%}_{-6.2\%}$ &   $86\%^{+4.9\%}_{-7.0\%}$ \\
       & Gradient &  $11\%^{+1.5\%}_{-1.3\%}$ &   $69\%^{+3.1\%}_{-3.3\%}$ \\
       & Integrated Gradient &  $25\%^{+2.6\%}_{-2.4\%}$ &   $86\%^{+1.0\%}_{-1.0\%}$ \\
\cline{1-4}
\multirow{3}{*}{bAbI-1} & Attention &  $84\%^{+4.8\%}_{-6.3\%}$ &  $100\%^{+0.3\%}_{-0.6\%}$ \\
       & Gradient &  $18\%^{+2.9\%}_{-2.6\%}$ &   $74\%^{+2.1\%}_{-2.3\%}$ \\
       & Integrated Gradient &  $28\%^{+3.4\%}_{-3.1\%}$ &   $85\%^{+3.4\%}_{-4.2\%}$ \\
\cline{1-4}
\multirow{3}{*}{bAbI-2} & Attention &  $74\%^{+4.6\%}_{-5.2\%}$ &   $99\%^{+0.4\%}_{-0.6\%}$ \\
       & Gradient &  $10\%^{+1.9\%}_{-1.6\%}$ &   $48\%^{+3.3\%}_{-3.3\%}$ \\
       & Integrated Gradient &  $12\%^{+1.9\%}_{-1.7\%}$ &   $51\%^{+3.9\%}_{-3.9\%}$ \\
\cline{1-4}
\multirow{3}{*}{bAbI-3} & Attention &  $60\%^{+6.1\%}_{-6.5\%}$ &   $98\%^{+0.7\%}_{-1.0\%}$ \\
       & Gradient &   $6\%^{+0.5\%}_{-0.5\%}$ &   $32\%^{+2.1\%}_{-2.0\%}$ \\
       & Integrated Gradient &   $8\%^{+1.4\%}_{-1.2\%}$ &   $37\%^{+4.1\%}_{-3.9\%}$ \\
\bottomrule
\end{tabular}

